Discrete-Time Adaptive Control of a Class of Nonlinear Systems Using High-Order Tuners

This paper concerns the adaptive control of a class of discrete-time nonlinear systems with all states accessible. Recently, a high-order tuner algorithm was developed for the minimization of convex loss functions with time-varying regressors in the context of an identification problem. Based on Nesterov's algorithm, the high-order tuner was shown to guarantee bounded parameter estimation when regressors vary with time, and to lead to accelerated convergence of the tracking error when regressors are constant. In this paper, we apply the high-order tuner to the adaptive control of a particular class of discrete-time nonlinear dynamical systems. First, we show that for plants of this class, the underlying dynamical error model can be causally converted to an algebraic error model. Second, we show that using this algebraic error model, the high-order tuner can be applied to provably stabilize the class of dynamical systems around a reference trajectory.

==> Old/2_problem_setting.tex <==
\section{PROBLEM SETTING} \label{sec:problem_setting}

% \begin{itemize}
%     \item Simplifications and assumptions
%     \item System: $x_i = Ax_{i-1} + bu_{i-1}$, $A$ unknown, $b$ known
%     \item Design feedback as $u_i = k_i^\top x_i$
%     \item Goal is to learn $k_i \rightarrow k_*$ such that $k_*$ stabilizes the system $(A, b)$
% \end{itemize}

% \subsection{System Identification}

% \begin{itemize}
%     \item Problem: $y_i = k_*^\top\phi_i$, $\phi_i$ and $y_i$ are given at every time step $i$, solve for $\theta_*$
%     \item Create an estimator: $\hat{y}_i = k_i^\top\phi_i$
%     \item Output error: $e_{yi} = \hat{y}_i - y_i = (k_i - k_*)^\top\phi_i = \tilde{k}_i^\top\phi_i$
% \end{itemize}

% \subsection{Adaptive Control of an LTI System as a System Identification Problem}

% \begin{itemize}
%     \item Reference model: $x_{mi} = A_mx_{m(i-1)} + br_{i-1}$
%     \item Error model 2: $e_i = A_me_{i-1} + b\tilde{k}_{i-1}^\top x_{i-1}$
%     \item Note: if $A_m$ is Schur-stable, then $e_i \rightarrow 0$ asymptotically as $\tilde{k}_i^\top x_i \rightarrow 0$
%     \item It is sufficient for adaptive control to ensure that $\tilde{k}_i^\top x_i \rightarrow 0$
%     \item Rearrange: $b^\top\Gamma(e_i - A_me_{i-1}) = b^\top\Gamma b\tilde{k}_{i-1}^\top x_{i-1}$
%     \item Define $e_{yi} = \frac{b^\top\Gamma(e_{i+1} - A_me_i)}{b^\top\Gamma b}$ and $\phi_i = x_i$
%     \item Error model 2 is equivalent to $e_{yi} = \tilde{k}_i^\top\phi_i$
%     \item Adaptive control is achieved if $e_{yi} \rightarrow 0$
% \end{itemize}

As described in Section \ref{sec:introduction}, we concern ourselves with the problem of adaptive control of the feedback-linearizable plant given in \eqref{eqn:plant}, where in general the linear dynamics and controls matrices are unknown and the nonlinear elements are known except for unknown coefficients. In order to simplify the proofs for the purposes of this paper, we make the following simplifications:
\begin{assumption} \label{asn:simplifications}
    We assume the following about the plant:
    \renewcommand{\labelenumi}{(\roman{enumi})}
    \begin{enumerate}
        \item The plant is single-input, i.e. $u_k \in \R$, $a_i \in \R^m$, \\ $B = b \in \R^n$
        \item $b$, the control vector, is known.
    \end{enumerate}
\end{assumption}
The simplified plant model is then given by
\begin{equation} \label{eqn:plant_simplified}
    x_{p(k+1)} = Ax_{pk} + b\Big(\sum_{i = 1}^N a_i^\top f_i(x_{pk}) + g(x_{pk})u_k\Big)
\end{equation}
\begin{remark} \label{rmk:simplifications}
    It is a moderately straightforward extension of this paper to extend the proofs in this paper to the case where $b$ is unknown and to the multi-input case where $B \in \R^{n \times m}$ (with different assumptions). See \cite{annaswamy_book} for methods.
\end{remark}

\subsection{The Adaptive Control Problem} \label{subsec:adaptive_control}

We take a model reference approach to adaptive control by proposing the reference model
\begin{equation} \label{eqn:reference_model}
    x_{m(k+1)} = A_mx_{mk} + br_k
\end{equation}
where $A_m$ is chosen by the control designer to be Schur-stable and $r_k$ is a bounded reference input. The goal is then to design linearizing feedback
\begin{equation} \label{eqn:optimal_feedback}
    u_k = \frac{1}{g(x_{pk})}\Big(k_*^\top x_{pk} - \sum_{i = 1}^N a_i^\top f_i(x_{pk}) + r_k\Big)
\end{equation}
such that the plant in \eqref{eqn:plant_simplified} behaves like the reference model in \eqref{eqn:reference_model}. Note that when $A$ and $a_i$ are known, setting $u_k$ as in \eqref{eqn:optimal_feedback} results in the system
\begin{equation} \label{eqn:plant_with_optimal_feedback}
    x_{p(k+1)} = (A + bk_*^\top)x_{pk} + br_k
\end{equation}
which behaves like the reference model if $A_m = A + bk_*^\top$.

When $A$ and $a_i$ are unknown, we cannot set $u_k$ directly to its optimal value in \eqref{eqn:optimal_feedback}. We therefore take a certainty equivalence approach: the control designer chooses a reference model governed by $A_m$, and the adaptive controller estimates $k_*$ and $a_i$ as $\hat{k}_k$ and $\hat{a}_{ik}$. Note that this approach assumes the existence of $k_*$ for the chosen $A_m$, even though $A$ is unknown when choosing $A_m$. This gives rise to the so-called matching condition:
\begin{assumption} \label{asn:matching_condition}
    We assume that there exists some $k_* \in \R^n$ such that
    \begin{equation} \label{eqn:matching_condition}
        A + bk_*^\top = A_m
    \end{equation}
\end{assumption}
\begin{remark} \label{rmk:matching_condition}
    This is a standard assumption in model-reference adaptive control when dealing with state-space systems. In the most general case when $A_m$ is designed with no information about $A$, the existence of $\theta_*$ must simply be assumed. In many practical settings, however, it may be that the structure of $A$ is known even if the precise values of its elements are not. \iffalse : for example, in controlling a quadrotor where the precise values of the principal moments of inertia are be unknown, it is still known where these values appear in $A$ and $B$. \fi In such cases, $A_m$ can be designed to ensure that the matching condition is satisfied.
\end{remark}

The goal of the controller is then to update the estimates $\hat{k}_k$ and $\hat{a}_{ik}$ at every time step so that the plant asymptotically behaves like the reference model. More concretely, defining the performance error
\begin{equation} \label{eqn:performance_error}
    e_k := x_{pk} - x_{mk}
\end{equation}
we can define the control objective:
\begin{definition} \label{def:stronger_objective}
    The control objective is met if
    \begin{equation} \label{eqn:stronger_objective}
        \lim_{k \rightarrow \infty} \|e_k\| = 0
    \end{equation}
\end{definition}

As has been thoroughly studied in existing literature, the model reference approach with certainty equivalence control is characterized by an error model, which describes how the performance error $e_k$ evolves with time. This error model is developed through the following process. At each time step, we use the current parameter estimates $\hat{k}_k$ and $\hat{a}_{ik}$ in the controller as follows:
\begin{equation} \label{eqn:feedback}
    u_k = \frac{1}{g(x_{pk})}\Big(\hat{k}_k^\top x_{pk} - \sum_{i = 1}^N \hat{a}_{ik}^\top f_i(x_{pk}) + r_k\Big)
\end{equation}
Applying \eqref{eqn:feedback} and \eqref{eqn:matching_condition} to \eqref{eqn:plant_simplified} and defining the parameter errors
\begin{equation} \label{eqn:parameter_error}
    \tilde{k}_k := \hat{k}_k - k_*, \,\, \tilde{a}_{ik} = \hat{a}_{ik} - a_i
\end{equation}
and rearranging, we obtain the restructured plant model:
\begin{equation} \label{eqn:plant_rearranged_1}
    x_{p(k+1)} = A_mx_{pk} + b\tilde{k}_k^\top x_{pk} - b\sum_{i = 1}^N\tilde{a}_{ik}^\top f_i(x_{pk}) + br_k
\end{equation}
Furthermore, defining the parameter error vector $\theta_k$ and regressor $\phi_k$ as
\begin{gather}
    \theta_k^\top = [\hat{k}_k^\top, \hat{a}_{1k}^\top, \dots, \hat{a}_{Nk}^\top] \label{eqn:theta} \\
    \phi_k^\top = [x_{pk}^\top, -f_1^\top(x_{pk}), \dots, -f_N^\top(x_{pk})] \label{eqn:phi}
\end{gather}
and defining $\theta_*$ and $\tilde{\theta}_k$ analogously, we simplify the plant model to the following.
\begin{equation} \label{eqn:plant_rearranged}
    x_{p(k+1)} = A_mx_{pk} + b\tilde{\theta}_k^\top\phi_k + br_k
\end{equation}
Finally, subtracting \eqref{eqn:reference_model} from \eqref{eqn:plant_rearranged} and applying \eqref{eqn:performance_error} gives the error model:
\begin{equation} \label{eqn:error_model_2}
    e_{k+1} = A_me_k + b\tilde{\theta}_k^\top\phi_k
\end{equation}

% \subsection{Noise Characteristics} \label{subsec:adaptive_control_noise}

% Let \{$\eta_k$\} be a stochastic process on probability space ($\Omega$, $\F$, $\mathbb{P}$).
% \begin{assumption} \label{asn:noise}
%     We assume that $\eta_k$ satisfies the following:
%     \renewcommand{\labelenumi}{(\roman{enumi})}
%     \begin{enumerate}
%         \item $\E(\eta_{k+1} | \F_k) = D_{k+1}$ a.s.
%         \item $\|d_{k+1}\| \leq D_{max} < \infty \,\, \forall k$ a.s.
%         \item $\Var(\eta_{k+1} | \F_k) = \Sigma_{k+1}$ a.s.
%         \item $\|\Sigma_{k+1}\| \leq \Sigma_{max} < \infty \,\, \forall k$ a.s.
%     \end{enumerate}
%     where $\F_k$ is a filtration on the sub-sigma increasing algebra group of $\sigma_k(\theta_1, ..., \theta_k)$ (i.e., the filtration $\F_k$ assumes we know all values of $\theta_i$ $\forall i \leq k$) \cite{QIN2020}.
% \end{assumption}

\subsection{Adaptive Control as a Linear Regression Problem} \label{subsec:linear_regression}

Using methods inspired by the work of Kudva and Narendra \cite{KN_law_paper_1} \cite{KN_law_paper_2}, we reframe the adaptive control problem as a linear regression problem with a time-varying regressor and output. Our motivation for doing this is the fact that the latter problem has been studied extensively, and reframing the adaptive control problem in this way allows us to build on that work.

We start by noting that because $A_m$ is Schur-stable, if $\tilde{\theta}_k^\top\phi_k$ goes to 0, then $e_k$ also goes to 0 asymptotically. Therefore, the control objective can be reframed as ensuring that $\tilde{\theta}_k^\top\phi_k \rightarrow 0$ as $k \rightarrow \infty$.

Equation \eqref{eqn:error_model_2} can be rewritten as
\begin{equation} \label{eqn:error_model_2_rearranged}
    \frac{b^\top\Gamma(e_{k+1} - A_me_k)}{b^\top\Gamma b} = \tilde{\theta}_k^\top\phi_k
\end{equation}
where $\Gamma > 0$ is any arbitrary positive definite matrix. We then define the prediction error
\begin{equation} \label{eqn:prediction_error}
    e_{y(k+1)} := \frac{b^\top\Gamma(e_{k+1} - A_me_k)}{b^\top\Gamma b}
\end{equation}
and the scalar output
\begin{equation} \label{eqn:output}
    y_{k+1} := \theta_*^\top\phi_k
\end{equation}
Note that \eqref{eqn:output} describes a linear regression model with $\phi_k$ as a time-varying regressor. Finally, as $\theta_k$ is defined as an estimator for $\theta_*$, we define an estimator for $y_{k+1}$ as
\begin{equation} \label{eqn:output_estimator}
    \hat{y}_{k+1} := \theta_k^\top\phi_k
\end{equation}
Taken together, \eqref{eqn:error_model_2_rearranged} - \eqref{eqn:output_estimator} describe the following online linear regression model:
\begin{equation} \label{eqn:linear_regression}
    \begin{gathered}
        y_{k+1} = \theta_*^\top\phi_k \\
        \hat{y}_{k+1} = \theta_k^\top\phi_k \\
        e_{y(k+1)} = \hat{y}_{k+1} - y_{k+1} = \tilde{\theta}_k^\top\phi_k
    \end{gathered}
\end{equation}

The relationship between the adaptive control problem and the linear regression problem in \eqref{eqn:linear_regression} is summarized in the following lemma.
\begin{lemma} \label{lem:error_models_1_2}
    If the prediction error $e_{y(k+1)}$ is bounded with $e_{y(k+1)} \in \ell_\infty$, then the performance error $e_k$ is also bounded with $\|e_k\| \in \ell_\infty$. Moreover, if
    \begin{equation}
        \lim_{k \rightarrow \infty} e_{y(k+1)} = 0
    \end{equation}
    then the control objective in \eqref{eqn:stronger_objective} is met.
\end{lemma}
\begin{proof}
    Equations \eqref{eqn:error_model_2} and \eqref{eqn:linear_regression} can be combined to yield
    \begin{equation} \label{eqn:error_model_2_1}
        e_{k+1} = A_me_k + be_{y(k+1)}
    \end{equation}
    If $e_{y(k+1)}$ is bounded, then \eqref{eqn:error_model_2_1} is a Schur-stable LTI system with a bounded input. It immediately follows that $\|e_k\|$ is bounded as well, concluding the first part of the proof.
    
    If moreover $e_{y(k+1)}$ tends to 0 asymptotically, then in the limit as $k \rightarrow \infty$, \eqref{eqn:error_model_2_1} reduces to $e_{k+1} = A_me_k$. Because $A_m$ is Schur-stable, it immediately follows that $e_k$ will tend to 0 asymptotically as well, meeting the control objective and concluding the second part of the proof.
\end{proof}
\begin{remark}
    Note that reframing the control problem as a linear regression problem would suggest that the goal is to solve for $\theta_*$, i.e. to ensure that $\theta_k \rightarrow \theta_*$ as $k \rightarrow \infty$. While achieving this ensures that the control objective is met (and is ideal for reasons of robustness as described in \cite{survey_paper}), this is not necessarily achievable unless $\{\phi_k\}_{k \geq 0}$ is persistently exciting (see \textbf{[cite a few things here]} for more information). However, as is well-known for many methods of updating $\theta_k$ and as we will show  for the high-order tuner as well, it is always possible to update $\theta_k$ in such a way that the error goes to 0 asymptotically. Therefore, the goal of the online linear regression problem is to update $\theta_k$ such that $e_{y(k+1)} \rightarrow 0$ as $k \rightarrow \infty$.
\end{remark}

The relationship between the error model in \eqref{eqn:error_model_2} and the linear regression model in \eqref{eqn:linear_regression} suggests Algorithm \ref{alg:adaptive_control}, a general algorithm for direct adaptive control of the class of systems covered in this paper. In the second-to-last line, ADAPTIVE\_LAW refers to any iterative algorithm for updating $\theta_k$. As we shall show in the following sections, update laws based on the gradient of a loss function such as normalized gradient descent and the high-order tuner lead to global stability, regardless of the initial parameter estimate $\theta_0$.

\begin{algorithm}[t]
  \caption{General Algorithm for Direct Adaptive Control of the Error Model in \eqref{eqn:error_model_2}}
  \label{alg:adaptive_control}
  \begin{algorithmic}[1]
    \STATE {\bfseries Input:} initial conditions $x_{p0}$, $x_{m0}$, initial parameter estimate $\theta_0$, reference input $\{r_k\}_{k \geq 0}$, reference system $(A_m, b)$, functions $f_1(\cdot), \dots, f_N(\cdot), g(\cdot)$, gain $\Gamma$, adaptive law gains
    \FOR{$k = 0, 1, 2, \ldots$}
    \STATE Let $\phi_0 = [x_{pk}^\top, -f_1(x_{pk}), \dots, -f_N(x_{pk})]^\top$
    \STATE \textbf{Receive} reference input $r_k$
    \STATE Let $u_k = \frac{1}{g(x_{pk})}(\theta_k^\top\phi_k + r_k)$
    \STATE \textbf{Apply} $u_k$ to plant
    \STATE \textbf{Measure} new state $x_{p(k+1)}$
    \STATE \textbf{Simulate} $x_{m(k+1)} = A_mx_{mk} + br_k$
    \STATE Let $e_{k+1} = x_{p(k+1)} - x_{m(k+1)}$
    \STATE Let $e_{y(k+1)} = \frac{b^\top\Gamma b(e_{k+1} - A_me_k)}{b^\top\Gamma b}$, \\
    $\hat{y}_{k+1} = \theta_k^\top x_{pk}$, \\
    $y_{k+1} = \hat{y}_{k+1} - e_{y(k+1)}$
    \STATE \textbf{Update} $\theta_{k+1} \leftarrow$ ADAPTIVE\_LAW$(\theta_k, *)$
    \ENDFOR
  \end{algorithmic}
\end{algorithm}

% \subsection{Linear Regression Noise Characteristics} \label{subsec:linear_regression_noise}

% Let \{$\eta_{yk}$\} be a stochastic process on probability space ($\Omega_y$, $\F_y$, $\mathbb{P}_y$).
% \begin{assumption} \label{asn:output_noise}
%     We assume that $\eta_{yk}$ satisfies the following:
%     \renewcommand{\labelenumi}{(\roman{enumi})}
%     \begin{enumerate}
%         \item $\E(\eta_{y(k+1)} | \F_{yk}) = d_{k+1}$ a.s.
%         \item $|d_{k+1}| \leq d_{max} < \infty \,\, \forall k$ a.s.
%         \item $\Var(\eta_{y(k+1)} | \F_{yk}) = \sigma^2_{k+1}$ a.s.
%         \item $\sigma^2_{k+1} \leq \sigma^2_{max} < \infty \,\, \forall k$ a.s.
%     \end{enumerate}
%     where $\F_{yk}$ is a filtration on the sub-sigma increasing algebra group of $\sigma_k(\theta_1, ..., \theta_k)$ (i.e., the filtration $\F_{yk}$ assumes we know all values of $\theta_i$ $\forall i \leq k$) \cite{QIN2020}.
% \end{assumption}
% \begin{remark} \label{rmk:output_noise}
%     This assumption follows naturally from Assumption \ref{asn:noise}.
% \end{remark}

==> layout.tex <==
\section{LAYOUT OF PAPER}

\subsection{Introduction}

A brief overview of the adaptive control problem, the direct adaptive control approach specifically, and the various adaptive laws.

Maybe also talk about persistent excitation? Not sure whether or not that should be within the scope of this paper.

\subsection{Problem Setting}

A more thorough overview of the problem setting.

\subsection{Adaptive Control Using First-Order Update Laws}

An overview and stability proof of the KN adaptive law, followed by a discussion of Goodwin's hyperplanes intuition and the single-projection adaptive law. (The stability proof of the latter is the same as the stability proof of the former.)

\subsection{The Double-Projection Algorithm as a High-Order Tuner}

Derivation and presentation of the double-projection adaptive law based on the intuition for the single-projection adaptive law.

\subsubsection{Connections to the High-Order Tuner Algorithm}

An explanation of how the double-projection adaptive law is related to the high-order tuner.

\subsubsection{Stability and Convergence}

A stability proof for the double-projection adaptive law, and discussion of simulation results.

\subsection{3rd-Order Tuners and Beyond}

A brief discussion of arbitrarily-high-order tuners -- no proofs, although I may offer a conjecture that for a system of any arbitrary size, there exists a tuner of sufficiently high order that will give constant-time control, and constant-time learning under finite excitation.

\subsection{Conclusions and Future Works}

Future works include an extension of the problem setting to the case where $b$ is unknown and to the multi-input case. We will also look at finite-time convergence rates and regret bounds, and consider higher-order tuners as well. 
